DPD-NeuralEngine: A 22-nm 6.6-TOPS/W/mm$^2$ Recurrent Neural Network Accelerator for Wideband Power Amplifier Digital Pre-Distortion

The increasing adoption of Deep Neural Network (DNN)-based Digital Pre-distortion (DPD) in modern communication systems necessitates efficient hardware implementations. This paper presents DPD-NeuralEngine, an ultra-fast, tiny-area, and power-efficient DPD accelerator based on a Gated Recurrent Unit (GRU) neural network (NN). Leveraging a co-designed software and hardware approach, our 22 nm CMOS implementation operates at 2 GHz, capable of processing I/Q signals up to 250 MSps. Experimental results demonstrate a throughput of 256.5 GOPS and power efficiency of 1.32 TOPS/W with DPD linearization performance measured in Adjacent Channel Power Ratio (ACPR) of -45.3 dBc and Error Vector Magnitude (EVM) of -39.8 dB. To our knowledge, this work represents the first AI-based DPD application-specific integrated circuit (ASIC) accelerator, achieving a power-area efficiency (PAE) of 6.6 TOPS/W/mm$^2$.

==> tabs/tab_compare.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}

\begin{table*}[!h]
\begin{minipage}{\textwidth}
\caption{Comparison with the State-of-the-Art DPD Hardware Accelerators and measured signal quality.}
\renewcommand{\arraystretch}{1.8}  % Increase row spacing
\fontsize{14}{16}\selectfont  % Increase font size to 12pt with 14pt line spacing
\label{tab:compare}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccccccccc|ccc}
\Xhline{6\arrayrulewidth}
 &
  \multicolumn{12}{c|}{\textbf{DPD Hardware Specification and Performance}} &
  \multicolumn{3}{c}{\textbf{Signal Config. and Quality\textsuperscript{1}}} \\ \hline
 &
  \begin{tabular}[c]{@{}c@{}}Architecture\\ ~\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Tech.\\ (nm)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Model\\ ~\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Precision\\(bits) ~\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}\#Param\\ ~\end{tabular} &
  \begin{tabular}[c]{@{}c@{}} OP/S\textsuperscript{2}\\ ~\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$\mathbf{f_{clk}}$\\ (MHz)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$\mathbf{f_{s, I/Q}}$\\ (MSps)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Latency\\ (ns)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Throughput\textsuperscript{2}\\ (GOPS)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Power\textsuperscript{3}\\ (W)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Efficiency\textsuperscript{2}\\ (GOPS/W)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}$\mathbf{f_{BB}}$\\ (MHz)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}ACPR \\ (dBc)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}EVM \\ (dB)\end{tabular} \\ \hline
This Work &
  ASIC &
  22 &
  RNN &
  W12A12 &
  502 &
  1,026 &
  2,000 &
  250 &
  \textbf{7.5} &
  256.5 &
  \textbf{0.20} &
  \textbf{1,315.4} &
  80 &
  -45.05 &
  -41.23 \\
~\cite{Huang2020} &
  FPGA (UltraScale+) &
  16 &
  GMP &
  W?A16 &
  36 &
  17 &
  300 &
  \textbf{2,400} &
  - &
  $\sim$40.8 &
  0.96 &
  $\sim$42.5 &
  400 &
  -44.7 &
  -39.2 \\
~\cite{Tommaso2022} &
  FPGA (Zynq-7000) &
  28 &
  MP &
  W?A16 &
  9 &
  30 &
  250 &
  250 &
  40 &
  $\sim$7.5 &
  0.23 &
  $\sim$32.6 &
  20 &
  -49.0 &
  - \\
~\cite{Yue2022} &
  FPGA (Virtex-7) &
  28 &
  GMP &
  W?A16 &
  38 &
  149 &
  - &
  400 &
  - &
  $\sim$59.6 &
  0.89 &
  $\sim$67.0 &
  100 &
  -46.45 &
  - \\
~\cite{li2024gpu} &
  GPU (RTX4080) &
  \textbf{5} &
  TDNN &
  FP32 &
  909 &
  $\sim$1,818 &
  $\sim$2,300 &
  1,000 &
  - &
  \textbf{$\sim$1,818} &
  $\leq$320 &
  $\geq$5.7 &
  200 &
  -45.2 &
  -35.34 \\
\Xhline{6\arrayrulewidth}
\end{tabular}
}

\vspace{1ex}
\footnotesize{\textsuperscript{1} These columns show the signal quality of PA outputs after applying DPD. However, their absolute values cannot be directly compared because each work uses different test signal configurations and PA hardware.} \\
\footnotesize{\textsuperscript{2} OP/S denotes Operations Per I/Q Sample (floating-point or fixed-point). GOPS (Giga Operations Per Second) is calculated as GOPS = OP/S $\times~f_{s, I/Q}$.} \\
\footnotesize{\textsuperscript{3} Total on-chip power, including dynamic and static power. Because~\cite{li2024gpu} did not report the measured power consumption of the RTX4080, we use its Thermal Design Power (TDP) instead~\cite{rtx4080}.} \\
% \footnotesize{\textsuperscript{4}~\cite{Huang2020} utilizes a parallel architecture with a parallelism factor of 8, resulting in the required operations per sample to \#OP/8.}

\end{minipage}
\end{table*}



==> tabs/tab_compare_asic.tex <==
\begin{table}[]
\caption{Comparison with Prior RNN/DNN ASICs}
\label{tab:compare_asic}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccccccc|c}
\Xhline{3\arrayrulewidth}
 &
  \cite{kadetotad20208} &
  \cite{shin201714} &
  \cite{kim202223} &
  \cite{lee2019} &
  \cite{Han2016} &
  \cite{Molendijk2023} &
  \cite{Lin2020} &
  \begin{tabular}[c]{@{}c@{}}This \\ work\end{tabular} \\ \hline
\begin{tabular}[c]{@{}c@{}}Technology\\  (nm)\end{tabular} &
  65 &
  65 &
  65 &
  65 &
  45 &
  22 &
  \textbf{7} &
  22 \\ \hline
\begin{tabular}[c]{@{}c@{}}$\mathrm{f}_{clk}$\\  (MHz)\end{tabular} &
  80&
  200&
  0.25 &
  200 &
  800 &
  300 &
  880 &
  \textbf{2,000}\\ \hline
\begin{tabular}[c]{@{}c@{}}Weight Prec.\\  (bits)\end{tabular} &
  32 &
  32 &
  32 &
  16 &
  4 &
  8 &
  8 &
  12 \\ \hline
\begin{tabular}[c]{@{}c@{}}Area \\ (mm\textsuperscript{2})\end{tabular} &
  7.7 &
  16.0 &
  0.4 &
  16 &
  40.8 &
  3.0 &
  3.0 &
  \textbf{0.2} \\ \hline
\begin{tabular}[c]{@{}c@{}}Supply \\ (V)\end{tabular} &
  1.1 &
  1.1 &
  0.75 &
  1.1 &
  - &
  0.5 &
  0.575 &
  0.9 \\ \hline
\begin{tabular}[c]{@{}c@{}}Power \\ (mW)\end{tabular} &
  67 &
  21 &
  \textbf{0.02} &
  297 &
  590 &
  31 &
  174 &
  195 \\ \hline
\begin{tabular}[c]{@{}c@{}}Throughput \\ (GOPS)\end{tabular} &
  165 &
  25 &
  0.004 &
  346 &
  102 &
  77 &
  \textbf{3,604} &
  257 \\ \hline
\begin{tabular}[c]{@{}c@{}}Power Efficiency \\ (TOPS/W)\end{tabular} &
  2.45 &
  1.19 &
  0.17 &
  3.08 &
  0.17 &
  2.47 &
  \textbf{6.83} &
  1.32 \\ \hline
\begin{tabular}[c]{@{}c@{}}Area Efficiency \\ (GOPS/mm\textsuperscript{2})\end{tabular} &
  21.3 &
  1.6 &
  0.01 &
  21.6 &
  2.5 &
  25.8 &
  1,185.7 &
  \textbf{1,282.5} \\ \hline
\begin{tabular}[c]{@{}c@{}}PAE \\ (TOPS/W/mm\textsuperscript{2})\end{tabular} &
  0.32 &
  0.07 &
  0.40 &
  0.07 &
  0.004 &
  0.83 &
  2.25 &
  \textbf{6.58} \\ 
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\end{table}





% \begin{table}[]
% \caption{Comparison with Conventional RNN Hardware Accelerators}
% \label{tab:compare_asic}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  &
%   \cite{kadetotad20208} &
%   \cite{shin201714} &
%   \cite{kim202223} &
%   \begin{tabular}[c]{@{}c@{}}This \\ work\end{tabular} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Technology\\  (nm)\end{tabular}$^\dagger$ &
%   65 &
%   65 &
%   65 &
%   22 \\ \hline
% \begin{tabular}[c]{@{}c@{}}$\mathrm{f}_{clk}$\\  (MHz)\end{tabular} &
%   80&
%   200&
%   0.25 &
%   2,000 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Area \\ (mm\textsuperscript{2})\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}7.74 \\ (0.89$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}16.00 \\ (1.83$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.43 \\ (0.05$^\dagger$)\end{tabular} &
%   \textbf{0.20} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Power \\ (mW)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}67.30 \\ (22.78$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}21.00 \\ (7.11$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.02 \\ (\textbf{0.008}$^\dagger$)\end{tabular} &
%   195.00 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Throughput \\ (GOPS)\end{tabular} &
%   164.95 &
%   25.00 &
%   0.004 &
%   \textbf{256.50} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Power Efficiency \\ (TOPS/W)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}2.45 \\ (\textbf{7.24}$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}1.19 \\ (3.52$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.17 \\ (0.51$^\dagger$)\end{tabular} &
%   1.32 \\ \hline
% \begin{tabular}[c]{@{}c@{}}Area Efficiency \\ (GOPS/mm\textsuperscript{2})\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}21.31 \\ (186.03$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}1.56 \\ (13.64$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.01 \\ (0.08$^\dagger$)\end{tabular} &
%   \textbf{1,282.50} \\ \hline
% \begin{tabular}[c]{@{}c@{}}PAE \\ (TOPS/W/mm\textsuperscript{2})\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.32 \\ (8.17$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.07 \\ (1.92$^\dagger$)\end{tabular} &
%   \begin{tabular}[c]{@{}c@{}}0.40 \\ (10.43$^\dagger$)\end{tabular} &
%   6.58 \\ \hline
% \end{tabular}
% }

% \vspace{1ex}

% \footnotesize{$^\dagger$Values normalized to 22 nm technology node.}

% \end{table}
